Where Does My Model Underperform? A Human Evaluation of Slice Discovery Algorithms

Machine learning (ML) models that achieve high average accuracy can still underperform on semantically coherent subsets ("slices") of data. This behavior can have significant societal consequences for the safety or bias of the model in deployment, but identifying these underperforming slices can be difficult in practice, especially in domains where practitioners lack access to group annotations to define coherent subsets of their data. Motivated by these challenges, ML researchers have developed new slice discovery algorithms that aim to group together coherent and high-error subsets of data. However, there has been little evaluation focused on whether these tools help humans form correct hypotheses about where (for which groups) their model underperforms. We conduct a controlled user study (N = 15) where we show 40 slices output by two state-of-the-art slice discovery algorithms to users, and ask them to form hypotheses about an object detection model. Our results provide positive evidence that these tools provide some benefit over a naive baseline, and also shed light on challenges faced by users during the hypothesis formation step. We conclude by discussing design opportunities for ML and HCI researchers. Our findings point to the importance of centering users when creating and evaluating new tools for slice discovery.

==> text/shared-sections/acknowledgements.tex <==
Sherry Tongshuang Wu
Valerie Chen
Vijay Viswanathan
Nupoor Gandhi
Luke Guerdan
Donald Bertucci




==> text/spurious-sections/conclusion.tex <==
\section{Conclusion}
Machine learning researchers have motivated new slice discovery algorithms as tools that can help users identify groups where their model underperforms.
From our controlled user study, we found positive evidence that existing algorithms may offer some benefit relative to a naive baseline of examining a random sample of errors.
However, our finding that coherence (i.e. the number of images that match the user's hypothesis) is \emph{not} predictive of the hypothesis's correctness directly challenges conventional wisdom that coherence is a valid proxy of utility.
Slice discovery researchers and users alike should keep in mind that even if \emph{many} images in an output slice match some description, this does not imply that the model underperforms on \emph{all} such images.
We hope our work sheds light on the complexities and exciting design challenges that emerge when we explicitly examine slicing not as the end goal, but rather a means to facilitate user understanding.


\newpage

==> text/spurious-sections/introduction.tex <==
\section{Introduction}

A growing number of works propose tools to help stakeholders to form hypotheses about the behavior of machine learning models.
One type of behavior that can have significant societal consequences occurs when a model underperforms on semantically coherent subsets (i.e. ``slices'') of data.
For example, \citet{buolamwini2018gender} found that leading tech companies' commercial facial recognition systems were significantly less accurate at classifying faces of women with darker skin.
Knowledge of this model behavior informed advocacy efforts that led to fundamental changes to dataset curation for facial recognition \citep{ibm2018response, birhane2022unseen} and public deliberation surrounding governance of facial recognition systems \citep{raji2022actionable}.
More broadly, knowledge of underperforming slices can inform model selection and deployment \citep{balayn2023faulty} or actions that can be taken to fix the model \citep{cabrera2021discovering, idrissi2022simple}.

\begin{figure*}[h]
\centering
\includegraphics[width=\linewidth]{figures/workflow.pdf}
\caption{An overview of the study in three steps.  (Left) We run different slice discovery algorithms to compute high-error slices (i.e. subsets of the input dataset).  (Middle) We conduct a human subject study where we \emph{show the slices from Step 1} to a human subject, who forms a hypothesis (i.e. description of a subgroup where the model underperforms) corresponding to each slice.  (Right) We validate each user-generated hypothesis from Step 2 by calculating the model's accuracy on a sample of images that match the user's description.}
\label{fig:experiment-phases}
\end{figure*}

However, identifying these underperforming slices can be difficult in practice.  
In many domains, practitioners often do not have access to labels that can be used to define semantically \emph{coherent} (i.e. united by a human-understandable concept) subsets of data.
Motivated by these challenges, machine learning researchers have developed new automated tools in the growing field of \emph{slice discovery}.
At a high level, these \emph{slice discovery algorithms} are unsupervised methods that aim to group together coherent and high-error slices of data \citep{ sohoni2020no, d2021spotlight, singla2021understanding, eyuboglu2022domino, plumb2023rigorous, wang2023error}.
These works propose that a human stakeholder can inspect the slices output by these algorithms to form hypotheses of model behavior, i.e. \emph{describe in words} a subgroup where the model underperforms.

While researchers continue to develop new slice discovery algorithms, there has been little evaluation of whether these algorithms help stakeholders achieve their proposed goals.
To bridge this gap, we return to the important human-centered task of understanding where (i.e. for which subgroups) a model underperforms.
Past evaluations have used subjective measures of the output slices' coherence (such as whether users can find a description that ``matches'' all the images in the slice) as \emph{proxies} of these algorithms' utility \citep{singla2021understanding, d2021spotlight}, but stop short of verifying whether these descriptions are useful or even correct depictions of the model.
In this work, we ask: \emph{Do the slices output by these algorithms help users form correct hypotheses of model behavior?}

As a motivating example, consider a scenario where a practitioner wishes to evaluate a new object detection model designed to be deployed in an autonomous vehicle.
The practitioner could run a slice discovery algorithm on a dataset of dash-cam photographs collected from field testing, but its output (groups of photos) is not immediately actionable.
Describing in words a group where the model underperforms (e.g. ``the model fails to identify stop signs in snowy environments'' \footnote{Scenario inspired by \citet{dunlap2023using}.}) is a prerequisite step for several downstream actions that the practitioner's company could take, such as initiating targeted data collection efforts (e.g. additional field testing to gather more data in snowy regions) or selective deployment (e.g. delaying roll-out of the new model in areas that experience snow).


However, taking action to address an \emph{incorrect} hypothesis can have several undesirable consequences.
For example, if the model actually performs just as well at detecting stop signs in snowy environments, then the company's efforts to improve the model's performance on that group may have been better invested elsewhere, or may even \emph{worsen} the model's performance on other groups \citep{li2022whac}.
Thus, we argue that this under-examined step of hypothesis formation is critically important for many stakeholders.

\textbf{Our Contributions.}  Several works propose that automated methods that return \emph{slices} of data assume that stakeholders can form valid behavioral hypotheses from inspecting the returned slices.
In this work, we examine this assumption by running a controlled user study ($N = 15$) with three parts, illustrated in Figure \ref{fig:experiment-phases}.
In the following sections, we provide an overview of slice discovery, motivate our research hypotheses and study design, and present results from our human subject evaluation.



==> text/spurious-sections/methodology.tex <==
\section{Experimental Design}

We present an overview of our research questions and study design (with complete details and screenshots of the study interface in Appendix \ref{apdx:study-design}).

\subsection{Research Questions}

Our primary research hypotheses measure the extent to which different slice discovery algorithms (\textsc{Domino} and \textsc{PlaneSpot}) achieve their proposed goals, relative to a naive baseline. 
First, we hypothesize that users' hypotheses corresponding to the slices output by algorithms \emph{designed for slice discovery} are more likely to be ``correct'':

\textbf{H1}.  A greater proportion of users' hypotheses corresponding to slices output by slice discovery algorithms will be correct, when compared to hypotheses corresponding to slices output by the naive baseline.

In addition to validating users' hypotheses, we also asked them to self-report how \emph{difficult} it was to form their hypothesis (i.e. describe the slice):

\textbf{H2}.  Users will rate slices output by slice discovery algorithms as \emph{easier to describe}, when compared to slices output by the naive baseline.

We also asked users to select all of the images that \emph{match their hypothesis} from a sample of the top-$20$ images that belong to the slice.
The number of matching images is one measure of the \emph{coherence} of the slice (i.e. the extent to which all of the images share a common description):

\textbf{H3}.  Users will \emph{select more images as ``matching'' their hypothesis} for slices output by slice discovery algorithms, when compared to slices output by the naive baseline.

Lastly, our final hypothesis studies whether coherence (when many images in the slice share a common description) implies correctness (that the model does in fact underperform on \emph{all} images that match this description):

\textbf{H4}.  The number of images that match a user's hypothesis (a measure of coherence) may not predict whether the hypothesis is correct.

\subsection{Study Design}

To conduct our study, we recruited $15$ participants who are current students that had self-reported ``intermediate knowledge in machine learning (ML) or computer vision (CV)''.
For the model $f$, we fine-tuned a pre-trained ResNet-18 on data from the MS-COCO \citep{lin2014microsoft}, a large-scale object detection task that we chose for its accessibility to a wide audience of non-expert stakeholders. 

We generated $60$ total slices ($20$ slices per each of the three algorithms described in Section \ref{sdm-prelims}) to show users. 
Rather than running each slice discovery algorithm on the \emph{entire} COCO test set (which contains $91$ object types), we ran each algorithm on subsets of the data that all have the same object (e.g., we give as input all images that have a ground-truth label of airplane).
We used each slice discovery algorithm to return the top $k = 4$ slices for $5$ different objects, chosen randomly from a list of candidate objects where the model had at least 50\% recall: \texttt{airplane}, \texttt{train}, \texttt{giraffe}, \texttt{skis}, and \texttt{broccoli}.

\textbf{Study Procedure.} 
After reading the study instructions and completing a walk-through of the study interface, users then were asked to complete a \emph{questionnaire} where they were asked to write down a behavioral hypothesis (i.e. describe in words a group that matches as many images in the slice as possible) for $12$ different slices.
Users were also asked to select all images in the slice that matched their hypothesis and rate how difficult it was for them to describe the slice.
We detail how we visualize the slices output by each algorithm and share the complete study questionnaire in Appendix \ref{apdx:procedure}.

\textbf{Experimental Design.} We showed each of the $60$ computed slices ($20$ per each of the $3$ algorithm ``conditions'') to $3$ different participants, collecting $3$ hypotheses per slice.
We used a within-subjects design, where each participant was randomly assigned to $3$ (out of $5$ candidate) object classes, but all participants were presented with slices computed by all $3$ different algorithms.
Users were blinded to the study condition when completing each questionnaire: they were not given any information about \emph{which algorithm} was used to compute each slice.


==> text/spurious-sections/results.tex <==
\section{Results}

To evaluate \textbf{H1} (whether the average number of correct hypotheses varies across conditions), we exclude hypotheses where we failed to find a sufficiently large sample of matching images to approximate the performance gap.
Applying this criteria, we retain $135$ out of the original $180$ hypotheses (75\%) where we found a sample of at least $15$ matching images.
To evaluate \textbf{H2} and \textbf{H3}, we calculate each measure using all $180$ of the original hypotheses.

To test for statistically significant differences between the three algorithm conditions, we ran ANOVA tests with Tukey post-hoc tests for multiple comparisons to compare the proportion of correct hypotheses (\textbf{H1}) and number of matching images (\textbf{H3}).  We ran Mann-Whitey tests with Bonferroni corrections to compare the Likert-scale self-reported difficulty of describing each slice (\textbf{H2}).  We used a $p$-value of $0.05$ as our cutoff for significance.
We present additional details for each statistical test (e.g. test statistics) and additional analyses in Appendix \ref{apdx:extended-results}.

\textbf{Correctness.}  For each condition, we calculated the proportion of hypotheses that are ``correct'' using a performance gap threshold of at least $20\%$.  
We observed that 51\% of all hypotheses (across all conditions) are correct (standard error 4.3\%).  When we stratify by condition, 35\% of \textsc{Baseline}, 49\% of \textsc{PlaneSpot}, and 72\% of \textsc{Domino} hypotheses are correct, with standard errors 6.7\%, 7.9\%, and 6.9\% respectively  (visualized in Figure \ref{fig:correctness}).
We found a statistically significant difference between the \textsc{Baseline} and \textsc{Domino} conditions only $(p < 0.001)$, partially supporting \textbf{H1}.
We present additional results where we ablate the performance gap threshold in Appendix \ref{apdx:correctness-ext}.
In summary, we found that a consistent trend (that \textsc{Domino} outperforms \textsc{PlaneSpot}, which outperforms \textsc{Baseline}) holds for all variations tried.


\textbf{Number of matching images.}  
Overall, we observed that users selected more images as ``matching'' their hypothesis for slices output by slice discovery algorithms relative to the naive baseline (supporting \textbf{H2}).
Figure \ref{fig:matching-images} shows the mean number of images (with standard error bars) and a strip plot to visualize the empirical distribution of matching images for different user hypotheses.
On average, users selected $12.9$ and $12.8$ out of the $20$ displayed images in the slice as ``matching'' their hypotheses for the \textsc{Domino}
and \textsc{PlaneSpot} conditions respectively (standard errors $0.57$ and $0.71$), vs. $8.8$ out of the $20$ images (standard error $0.60$) for the \textsc{Baseline} hypotheses.
We observed significant pairwise differences between the two slice discovery conditions vs. the baseline condition (with $p < 0.0001$ for both \textsc{Domino} and \textsc{PlaneSpot}), and no significant difference between the two slice discovery conditions.
However, we note that while the \emph{average} number of matching images (across all hypotheses) is higher for both slice discovery conditions, there is still high \emph{variance} across hypotheses.
%For example, 30\% of hypotheses from the \textsc{Domino} or \textsc{PlaneSpot} conditions had $9$ or fewer matching images (out of $20$), compared to 65\% of hypotheses from the baseline condition.

\textbf{Self-reported Difficulty.}  Overall, we observed that users rated slices output by the slice discovery algorithms as being \emph{easier to describe} compared to slices output by the naive baseline condition (supporting \textbf{H3}).  
Figure \ref{fig:reported-difficulty} shows the average difficulty rating and a histogram of Likert-scale ratings for each condition.  We observed significant pairwise differences between the two slice discovery conditions vs. the baseline ($p < 0.0001$), and no significant difference between the two slice discovery conditions.  

\textbf{Does coherence imply correctness?}  To examine whether coherence (i.e. the number of images in the slice that match a hypothesis) is an appropriate proxy of the hypothesis's  correctness (\textbf{H4}), we ran two Spearman's rank correlation tests.
For both tests, the independent variable is the number of matching images.
We tried two dependent variables: the value of the approximate performance gap for the hypothesis (defined in Equation \ref{eqn:gap}), and an indicator for hypothesis correctness using performance gap threshold $\tau = 0.2$.
For these analyses only, we retained only the hypotheses that corresponded to slices output by slice discovery algorithms (i.e. slices that were designed to be coherent), and excluded slices output by the baseline condition.

We found \emph{no significant association} between the number of images that match each hypothesis and its correctness, supporting \textbf{H4}. 
For both dependent variables, the number of matching images is only weakly correlated with the hypothesis's correctness, with correlation coefficients $r_s = 0.05$ with $p = 0.6194$ for the value of the performance gap, and $r_s = 0.07$ with $p = 0.5027$ for the correctness indicator.
When we examined the hypotheses that had the highest number of matching images (at least 15 out of 20), only 59\% of these hypotheses were correct, a rate \emph{lower} than the overall base rate of 61\% accuracy for all hypotheses.
%- just because the user can come up with a valid description that ``matches'' the slice, does not mean that the model indeed underperforms on it

==> text/spurious-sections/slice-overview.tex <==
\section{Slice Discovery Preliminaries}\label{sdm-prelims}

We focus our study on \emph{slice discovery algorithms}: fully automated methods that aim to partition the data into coherent and high-error subsets \citep{ eyuboglu2022domino, plumb2023rigorous}.  We exclude methods that rely on additional information such as labels \citep{liu2021just} or human supervision \citep{cabrera2023zeno, suresh2023kaleidoscope} to define coherent subsets.  
Consequently, the methods we study \emph{do not} require the practitioner to anticipate the types of inputs where the model may underperform in advance \citep{d2021spotlight}.

\textbf{Definition.}  We follow \citet{plumb2023rigorous} and define a slice discovery algorithm as a method that given as input a trained model $f$ and dataset of labeled images $D = \{(x_i, y_i) \}_{i = 1}^n$\footnote{We follow past work and give a separate hold-out test set that the model $f$ was \emph{not} trained on as the input to a slice discovery algorithm.}, outputs $k$ slices $\left[ \Psi_j \right]_{j = 1}^k$.  
Each slice $\Psi_j \subseteq D$ is a subset of the data.
The goal of slice discovery is for each slice $\Psi_j$ to correspond to a \emph{single coherent subgroup where the model indeed underperforms} (i.e. $f$ has lower accuracy for images in $\Psi_j$ than for all images in $D$).
Past works propose that a practitioner can manually inspect the datapoints belonging to each slice to ``identify common attributes'' \citep{eyuboglu2022domino} to describe the underperforming subgroups.

\textbf{Methods.}
We evaluate two existing slice discovery algorithms: \textsc{Domino} \citep{eyuboglu2022domino} and \textsc{PlaneSpot} \citep{plumb2023rigorous}.  
Both algorithms work by running error-aware clustering on an embedding of each image.  
They differ in the specific clustering algorithm and embedding that they use.
We provide an extended description of each algorithm in Appendix \ref{apdx:sdms-extended}.
We chose to evaluate these two algorithms because they achieved state-of-the-art performance on past benchmarks at the time we ran our study.

Our \textsc{Baseline} algorithm randomly samples from the set of all misclassified images without replacement.
While a subset of random misclassified images is high-error, it is unlikely to be coherent.
Our baseline was designed to simulate a naive workflow where a practitioner simply inspects an (unsorted) sample of errors to form hypotheses.

\textbf{Validating User Hypotheses.}
To evaluate each slice discovery algorithm, our study focuses on the human-centered task of \emph{hypothesis formation}.
We define a ``\emph{hypothesis}'' as a \emph{user-generated text description} of a group where they believe that the model underperforms.
Intuitively, a ``correct hypothesis'' should describe a group where the model has significantly lower accuracy.
If $\Phi$ denotes the set of all images in $D$ that belong to the group, we define the \emph{performance gap} $Gap(f, \Phi)$ of $f$ on $\Phi$ as
\begin{equation}
         \underbrace{\frac{1}{| D | } \sum_{(x, y) \in D } \mathbbm{1}(f(x) = y)}_{\text{average accuracy on $D $}} - \underbrace{\frac{1}{| \Phi| } \sum_{(x, y) \in \Phi} \mathbbm{1}(f(x) = y)}_{\text{average accuracy on $\Phi \subset D$}}
\label{eqn:gap}
\end{equation}

We define the correctness of the hypothesis ``$f$ underperforms on $\Phi$'' by thresholding the gap:
$Gap(f, \Phi) \geq \tau$. 
If we set $\tau = 0.2$, then a ``correct'' hypothesis describes a group where the model has 20\% worse average accuracy on images that belong to the group.

However, in many settings, we do not have access to $\Phi$, the complete set of images in $D$ that match each hypothesis.
Therefore, we decided to \emph{approximate} the model's performance gap for each hypothesis using a sample $\hat{\Phi}$ of images that match each hypothesis, where $\hat{\Phi} \subset \Phi$. 
To retrieve $\hat{\Phi}$, we followed past work \citep{gao2022adaptive} and ranked candidate images using their \emph{CLIP similarity score} \citep{radford2021learning} to the hypothesis text description.
We then manually annotated whether each retrieved image matched the user's hypothesis.
We provide an extended description of our approximation strategy in Appendix \ref{apdx:clip-retrieval}.

